GoSafeOpt: Scalable Safe Exploration for Global Optimization of Dynamical Systems

Learning optimal control policies directly on physical systems is challenging since even a single failure can lead to costly hardware damage. Most existing model-free learning methods that guarantee safety, i.e., no failures, during exploration are limited to local optima. A notable exception is the GoSafe algorithm, which, unfortunately, cannot handle high-dimensional systems and hence cannot be applied to most real-world dynamical systems. This work proposes GoSafeOpt as the first algorithm that can safely discover globally optimal policies for high-dimensional systems while giving safety and optimality guarantees. We demonstrate the superiority of GoSafeOpt over competing model-free safe learning methods on a robot arm that would be prohibitive for GoSafe.

==> preamble.tex <==
\RequirePackage{amsthm}
\usepackage{booktabs}
\usepackage{multirow}
\RequirePackage{amssymb}
\RequirePackage{setspace}
\usepackage{hyperref}
\theoremstyle{plain}
\usepackage{comment}
\usepackage{enumitem}
\hypersetup{hidelinks}
\usepackage{thm-restate}
\makeatletter
\newcommand{\myitem}[1]{%
\item[#1]\protected@edef\@currentlabel{#1}%
}
\makeatother
\usepackage[margin=1in]{geometry}
\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{observation}[theorem]{Observation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{example}[theorem]{Example}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newcommand{\safeopt}{\textsc{SafeOpt}\xspace}
\newcommand{\gosafe}{\textsc{GoSafe}\xspace}
\newcommand{\gosafeopt}{\textsc{GoSafeOpt}\xspace}
\newcommand{\safeoptswarm}{\textsc{SafeOptSwarm}\xspace}
\newcommand{\capt}[1]{\mdseries{\emph{#1}}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\xdes}{\ensuremath{x_{\mathrm{des}}(t)}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\N}{\ensuremath{\mathcal{N}}}
\newcommand{\conset}{\ensuremath{\{1,\dots,q\}}}
\newcommand{\traj}[3]{\xi_{(#1,#2,#3)}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert_1}
\newcommand{\normAny}[1]{\left\lVert#1\right\rVert}
\newcommand{\normgeneral}[2]{\left\lVert#1\right\rVert_#2}
\newcommand{\G}{\ensuremath{\mathcal{G}_n}}
\newcommand{\M}{\ensuremath{\mathcal{M}_n}}
\newcommand{\idxk}{
% "Tighter" index k
\hspace{-0.5pt}(t)\hspace{0.5pt}
}

\newcommand{\idxkmo}{
% "Tighter" index k-1
\hspace{-0.5pt}(t\scalebox{0.75}[1.0]{\(-\)}\Delta t)\hspace{0.5pt}
}
\newcommand{\idxkma}{
% "Tighter" index k-1
\hspace{-0.5pt}(t\scalebox{0.75}[1.0]{\(+\)}\Delta t)\hspace{0.5pt}
}
\newcommand{\fakepar}[1]{\vspace{1mm}\noindent\textit{#1.}} 
\newcommand{\heading}[1]{\vspace{1mm}\noindent\textit{#1}}
\newcommand{\extranote}{\vspace{1mm}\noindent\textit{Remark}: }
\newcommand{\headingBold}[1]{\vspace{1mm}\noindent#1}
\usepackage{amsmath}
\DeclareMathOperator{\Rcon}{\ensuremath{R_\epsilon^\mathrm{c}}}
\DeclareMathOperator{\Rglob}{\ensuremath{R_\epsilon}}
\DeclareMathOperator*{\argmax}{arg\,max}
\usepackage{thmtools}
\usepackage{thm-restate}
\declaretheorem[style=plain]{Theorem}
\usepackage[symbols]{glossaries-extra}
\makenoidxglossaries
\setabbreviationstyle{long-short}% glossaries-extra.sty
\newabbreviation{BO}{BO}{Bayesian optimization}
\newabbreviation{RL}{RL}{reinforcement learning}
\newabbreviation{DOF}{DOF}{degree of freedom}
\newabbreviation{MDP}{MDP}{Markov decision process}
\newabbreviation{CMDP}{CMDP}{constrained Markov decision process}
%\newabbreviation{GP}{GP}{Gaussian process}
% Consider using this instead
%\newacronym[\glslongpluralkey={Gaussian processes}]{GP}{GP}{Gaussian process}
\newacronym[plural=GPs,firstplural=Gaussian processes (GPs)]{GP}{GP}{Gaussian process}

%\newabbreviation{GPs}{GPs}{Gaussian processes}
\newabbreviation{AI}{AI}{artificial intelligence}
\newabbreviation{GPR}{GPR}{Gaussian process regression}
\newabbreviation{RKHS}{RKHS}{reproducing kernel Hilbert space}
\newabbreviation{wlog}{w.l.o.g}{without loss of generality}
\newabbreviation{iid}{i.i.d.}{independent and identically distributed}
\newabbreviation{ucb}{GP-UCB}{GP-upper confidence bound}
\newabbreviation{pso}{PSO}{particle swarm optimization}
\newabbreviation{se}{SE}{squared exponential}
\newabbreviation{lqr}{LQR}{linear-quadratic regulator}
\glsxtrnewsymbol [description={policy parameter}]{policyparam}{\ensuremath{a}}% symbol
\glsxtrnewsymbol [description={state vector}]{statevec}{\ensuremath{x(t)}}% symbol
\glsxtrnewsymbol [description={desired state}]{statedes}{\xdes}% symbol
\glsxtrnewsymbol [description={Initial State}]{x0}{\ensuremath{x_0}}
\glsxtrnewsymbol [description={applied input}]{input}{\ensuremath{u(t)}}
\glsxtrnewsymbol [description={constraints indices}]{conset}{\ensuremath{\mathcal{I}_g}}
\glsxtrnewsymbol [description={state space}]{statespace}{\ensuremath{\mathcal{X}}}
\glsxtrnewsymbol [description={parameter space}]{actionspace}{\ensuremath{\mathcal{A}}}
\glsxtrnewsymbol [description={discretized state space}]{statespacediscrete}{\ensuremath{\mathcal{X}_{\mu}}}
\glsxtrnewsymbol[description={one-step reachability operator}]{rcon}{\ensuremath{\Rcon}}
\glsxtrnewsymbol[description={maximizer set}]{Mn}{\M}
\glsxtrnewsymbol[description={expander set}]{Gn}{\G}
\newabbreviation{eic}{EIC}{expected improvement with constraints}
\newabbreviation{LSE}{\textbf{LSE}}{local safe exploration}
\newabbreviation{LSEP}{\textbf{LSE-P}}{local safe exploration in parameter space}
\newabbreviation{LSEPS}{\textbf{LSE-PS}}{Local safe exploration in the joint parameter and state space}
\newabbreviation{GE}{\textbf{GE}}{global exploration}
\def\textmarker#1#2{\textcolor{#1}{#2}}%*%
\newtheorem*{remark}{Remark}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem*{definition}{Definition}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}


